AmaSQuAD: A Benchmark for Amharic Extractive Question Answering

This research presents a novel framework for translating extractive question-answering datasets into low-resource languages, as demonstrated by the creation of the AmaSQuAD dataset, a translation of SQuAD 2.0 into Amharic. The methodology addresses challenges related to misalignment between translated questions and answers, as well as the presence of multiple answer instances in the translated context. For this purpose, we used cosine similarity utilizing embeddings from a fine-tuned BERT-based model for Amharic and Longest Common Subsequence (LCS). Additionally, we fine-tune the XLM-R model on the AmaSQuAD synthetic dataset for Amharic Question-Answering. The results show an improvement in baseline performance, with the fine-tuned model achieving an increase in the F1 score from 36.55% to 44.41% and 50.01% to 57.5% on the AmaSQuAD development dataset. Moreover, the model demonstrates improvement on the human-curated AmQA dataset, increasing the F1 score from 67.80% to 68.80% and the exact match score from 52.50% to 52.66%.The AmaSQuAD dataset is publicly available Datasets

==> sections/futurework.tex <==
\section{Future Works}
In future research, several avenues could be explored to enhance the performance and applicability of question-answering models for Amharic. Firstly, various adjustments of weights (w1 and w2) for cosine similarity and LCS for Algorithm 1 to locate the translated answer from the translated context should be investigated for the extraction process. Human evaluations should also provide feedback on the quality of the AmSQuAd dataset. Additionally, there is a need to address the limitations of current datasets, such as the absence of unanswerable questions and the relatively small size of datasets like AmQA. Incorporating unanswerable questions and expanding dataset sizes would provide a more realistic evaluation of model capabilities. Furthermore, future studies could investigate the impact of pre-training on larger Amharic corpora using diverse pre-training strategies, as demonstrated in recent work. These efforts could lead to significant advancements in question-answering systems.
